Unified 3D Mesh Recovery of Humans and Animals by Learning Animal Exercise

We propose an end-to-end unified 3D mesh recovery of humans and quadruped animals trained in a weakly-supervised way. Unlike recent work focusing on a single target class only, we aim to recover 3D mesh of broader classes with a single multi-task model. However, there exists no dataset that can directly enable multi-task learning due to the absence of both human and animal annotations for a single object, e.g., a human image does not have animal pose annotations; thus, we have to devise a new way to exploit heterogeneous datasets. To make the unstable disjoint multi-task learning jointly trainable, we propose to exploit the morphological similarity between humans and animals, motivated by animal exercise where humans imitate animal poses. We realize the morphological similarity by semantic correspondences, called sub-keypoint, which enables joint training of human and animal mesh regression branches. Besides, we propose class-sensitive regularization methods to avoid a mean-shape bias and to improve the distinctiveness across multi-classes. Our method performs favorably against recent uni-modal models on various human and animal datasets while being far more compact.

==> figure_tex/subkpt_table.tex <==
\begin{wrapfigure}{R}{0.4\textwidth}
\centering
% \framebox{\rule{0pt}{2in}{} \rule{0.9\linewidth}{0pt}}
%   \includegraphics[width=0.5\textwidth]{figure_tex/figures/subkeypointA_v4.pdf}
    \includegraphics[width=0.3\textwidth]{figure_tex/figures/subkeypointB_v2.pdf}

  \caption{Sub-keypoint groups and corresponding pairs}
\label{fig:subkpt_body}
\end{wrapfigure}

==> tables/table_ablation.tex <==
% \begin{table}[t]
%     \centering
%     \begin{tabularx}{\columnwidth}{@{} cc ccccccc c@{}} 
%     \toprule
%         & & \multicolumn{6}{ c }{{\bfseries Labels of Sub-Keypoints}} \\ 
%         \cmidrule(l){3-8} \cmidrule(l){9-10}
%         \multicolumn{2}{c}{\# of Subkpt}
%         & \multicolumn{1}{P}{Ey}
%         & \multicolumn{1}{P}{Ank}  
%         & \multicolumn{1}{P}{Wr} 
%         & \multicolumn{1}{P}{Sh}
%         & \multicolumn{1}{P}{El}
%         & \multicolumn{1}{P}{No}
%         & \multicolumn{2}{c}{PCK [\%] $\uparrow$}\\ 
%         \midrule
%         \multicolumn{2}{c}{15} & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \multicolumn{2}{c}{73.16}\\ 
%         \multicolumn{2}{c}{\textbf{10}} & \checkmark & \checkmark & \checkmark & \checkmark & & & \multicolumn{2}{c}{\textbf{73.23}}\\ 
%         \multicolumn{2}{c}{6}  & \checkmark & \checkmark & \checkmark & & & & \multicolumn{2}{c}{72.14}\\ 
%         \multicolumn{2}{c}{0}  & & & & & & & \multicolumn{2}{c}{?}\\ 
%     \bottomrule
%     \end{tabularx}
%     \vspace{1mm}
%     \caption{Ablation study on the method and number of sub-keypoints used in the loss. Evaluated on Stanford Extra dataset. The numbers are mean percentage of correct keypoints (PCK) in \%.}
% \label{table:subkpt}
% \end{table}

% \begin{table}[t]
%     \centering
%     \resizebox{\columnwidth}{!}{
%         \begin{tabular}{cc}
%             \begin{minipage}{0.68\columnwidth}
%             \centering
%                 % \begin{tabular}{l c}
%                 \begin{tabularx}{\columnwidth}{@{} cc cccccc c@{}} 
%                 \toprule
%                      & & \multicolumn{5}{ c }{{\bfseries Labels of Sub-Keypoints}} & Dog\\ 
%                     \cmidrule(lr){3-7}
%                     \multicolumn{2}{c}{\# of Subkpt}
%                     & Eyes & BL & TL & ML & Nose
%                     & \multicolumn{2}{c}{PCK [\%] $\uparrow$}\\ 
%                     \midrule
%                     \multicolumn{2}{c}{15} & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \multicolumn{2}{c}{73.16}\\
%                     \multicolumn{2}{c}{\textbf{10}} & \checkmark & \checkmark & \checkmark & & & \multicolumn{2}{c}{\textbf{\underline{73.23}}}\\ 
%                     \multicolumn{2}{c}{6}  & \checkmark & \checkmark & & & & \multicolumn{2}{c}{72.14}\\ 
%                     \multicolumn{2}{c}{0}  & & & & & & \multicolumn{2}{c}{?}\\ 
%                 \bottomrule
%                 \end{tabularx}%
%                 \vspace{1mm}
%                 \caption{Ablation study on the number of sub-keypoints.}
%                 \label{table:ablation:subkpt}
%             \end{minipage} &
        
%             \begin{minipage}{0.68\columnwidth}
%             \centering
%                 \begin{tabularx}{\columnwidth}{cc ccccc c} 
%                 \toprule
%                     & & \multicolumn{4}{ c }{{\bfseries Number of datasets available}} & \\ 
%                     \cmidrule(l){3-6}
%                   \multicolumn{2}{c}{Dataset \#}& Human & Dog & Horse & Cow & PCK [\%] $\uparrow$\\ 
%                     \midrule
%                     \multicolumn{2}{c}{0.6k} & 0.3k & 0.3k & & & 40.83\\ 
%                     \multicolumn{2}{c}{1.2k} & 0.3k & 0.3k & 0.3k & 0.3k & 48.07\\ 
%                     \multicolumn{2}{c}{1.0k} & 0.3k & 0.1k & 0.3k & 0.3k & 38.50\\ 
%                     \multicolumn{2}{c}{1.2k} & 0.5k & 0.1k & 0.3k & 0.3k & 43.64\\ 
%                 \bottomrule
%                 \end{tabularx}%
%                 \vspace{1mm}
%                 \caption{Data efficiency experiments on Stanford Extra dataset.}
%                 \label{table:ablation:dataset}
%             \end{minipage}
%         \end{tabular}
%     }
% \end{table}

\begin{table}[t]
    \centering
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{cc}
            \begin{minipage}{0.73\columnwidth}
            \centering
                % \begin{tabular}{l c}
                \begin{tabular}{cc ccccc cc} 
                \toprule
                     & & \multicolumn{5}{ c }{{\bfseries Labels of Sub-Keypoints}} &\multicolumn{2}{c}{Class: Dog}\\ 
                    \cmidrule(lr){3-7}
                    \multicolumn{2}{c}{\# of Subkpt}
                    & Eyes & BL & TL & ML & Nose
                    & \multicolumn{2}{c}{PCK [\%] $\uparrow$}\\ 
                    \midrule
                    \multicolumn{2}{c}{15} & \ccy{\checkmark} & \ccy{\checkmark} & \cco{\checkmark} & \ccr{\checkmark} & \ccr{\checkmark} & \multicolumn{2}{c}{73.16}\\
                    \multicolumn{2}{c}{\textbf{10}} & \ccy{\checkmark} & \ccy{\checkmark} & \cco{\checkmark} & & & \multicolumn{2}{c}{\textbf{\underline{73.23}}}\\ 
                    \multicolumn{2}{c}{6}  & \ccy{\checkmark} & \ccy{\checkmark} & & & & \multicolumn{2}{c}{72.14}\\ 
                    \multicolumn{2}{c}{0}  & & & & & & \multicolumn{2}{c}{71.89}\\ 
                \bottomrule
                \end{tabular}%
                \vspace{1mm}
                \caption{Ablation study on the number of sub-keypoints.}
                \label{table:ablation:subkpt}
            \end{minipage} &
        
            \begin{minipage}{0.73\columnwidth}
            \centering
                 \begin{tabular}{cc ccccc c} 
                \toprule
                    & & \multicolumn{4}{ c }{{\bfseries Number of datasets available}} &\multicolumn{2}{c}{Class: Dog}\\ 
                    \cmidrule(l){3-6}
                  \multicolumn{2}{c}{Dataset \#}& Human & Dog & Horse & Cow & PCK [\%] $\uparrow$\\ 
                    \midrule
                    \multicolumn{2}{c}{0.6k} & 0.3k & 0.3k & & & 40.83\\ 
                    \multicolumn{2}{c}{1.2k} & 0.3k & 0.3k & 0.3k & 0.3k & 48.07\\ 
                    \multicolumn{2}{c}{1.0k} & 0.3k & 0.1k & 0.3k & 0.3k & 38.50\\ 
                    \multicolumn{2}{c}{1.2k} & 0.5k & 0.1k & 0.3k & 0.3k & 43.64\\ 
                \bottomrule
                \end{tabular}%
                \vspace{1mm}
                \caption{\small{Sample efficiency experiments on Stanford Extra dataset.}}
                \label{table:ablation:dataset}
            \end{minipage}
        \end{tabular}
    }
\end{table}
